Extended X-ray emission associated with the radio lobes and the environments of 60 radio galaxies

This paper studied the faint, diffuse extended X-ray emission associated with the radio lobes and the hot gas in the intracluster medium (ICM) environment for a sample of radio galaxies. We used shallow ($\sim 10$ ks) archival Chandra observations for 60 radio galaxies (7 FR I and 53 FR II) with $0.0222 \le z \le 1.785$ selected from the 298 extragalactic radio sources identified in the 3CR catalog. We used Bayesian statistics to look for any asymmetry in the extended X-ray emission between regions that contain the radio lobes and regions that contain the hot gas in the ICM. In the Chandra broadband ($0.5 - 7.0$ keV), which has the highest detected X-ray flux and the highest signal-to-noise ratio, we found that the non-thermal X-ray emission from the radio lobes dominates the thermal X-ray emission from the environment for $\sim 77\%$ of the sources in our sample. We also found that the relative amount of on-jet axis non-thermal emission from the radio lobes tends to increase with redshift compared to the off-jet axis thermal emission from the environment. This suggests that the dominant X-ray mechanism for the non-thermal X-ray emission in the radio lobes is due to the inverse Compton upscattering of cosmic microwave background (CMB) seed photons by relativistic electrons in the radio lobes, a process for which the observed flux is roughly redshift independent due to the increasing CMB energy density with increasing redshift.

==> count_rates.tex <==
\begin{deluxetable*}{lcccc}
\centering
\tablecolumns{12} 
\tablewidth{700pt}
\tabletypesize{\small}
\tablecaption{\sout{Predicted count rates using the X-ray simulation tool, \texttt{PIMMS}. This example shows the expected count rates for the first source in the sample, 3C16, for different bands assuming a power law and Raymond-Smith (RS) thermal plasma model. The power law count rate exceeds the RS count rate in the soft band. However, the power law index is steeper than the RS model, so the count rate between the two becomes roughly comparable in the medium band. The RS count rate exceeds the power law in the hard band. The broad band is dominated by the power law model. The count-rate estimator provided similar results when ran on other sources in our sample.}}\label{tab:count_rates}
\label{tab:six}
\tablehead{ 
\colhead{\sout{Band}} & \colhead{\sout{Power law}\tablenotemark{a}} & \colhead{\sout{RS}\tablenotemark{b}} & \colhead{\sout{RS}} & \colhead{\sout{RS}} \\
\colhead{} & \colhead{\sout{($\alpha = 0.7$)}} & \colhead{\sout{($T = 10^{6.7}$ K)}} & \colhead{\sout{($T = 10^{7.0}$ K)}} & \colhead{\sout{($T = 10^{7.5}$ K)}}
}
\startdata 
\sout{Soft} & \sout{3.56E-4} & \sout{7.54E-5} & \sout{1.55E-4} & \sout{2.94E-4} \\
\sout{Medium} & \sout{9.64E-4} & \sout{9.46E-4} & \sout{9.47E-4} & \sout{9.65E-4} \\
\sout{Hard} & \sout{1.70E-3} & \sout{3.36E-3} & \sout{3.11E-3} & \sout{2.63E-4} \\
\sout{Broad} & \sout{2.82E-3} & \sout{8.78E-4} & \sout{2.30E-3} & \sout{4.30E-4} \\
\enddata 
\tablenotetext{a}{\sout{Estimated X-ray count rate on the \textit{Chandra} ACIS-S chip assuming a power law model ($f_{\nu} \sim \nu^{- \alpha}$) with $\alpha$ = 0.7.}}
\tablenotetext{b}{\sout{Estimated X-ray count rate on the \textit{Chandra} ACIS-S chip  assuming the Raymond-Smith \mbox{\citep{raymond_smith}} thermal plasma model for $T$ = 10$^{6.7}$ K, 10$^{7.0}$ K, and 10$^{7.5}$ K.}}
\end{deluxetable*} 
